Cosmic flows in the nearby Universe: new peculiar velocities from SNe and cosmological constraints

The peculiar velocity field offers a unique way to probe dark matter density field on large scales at low redshifts. In this work, we have compiled a new sample of 465 peculiar velocities from low redshift $(z < 0.067)$ Type Ia supernovae. We compare the reconstructed velocity field derived from the 2M++ galaxy redshift compilation to the supernovae, the SFI++ and the 2MTF Tully-Fisher distance catalogues. We used a forward method to jointly infer the distances and the velocities of distance indicators by comparing the observations to the reconstruction. Comparison of the reconstructed peculiar velocity fields to observations allows us to infer the cosmological parameter combination $f\sigma_8$, and the bulk flow velocity arising from outside the survey volume. The residual bulk flow arising from outside the 2M++ volume is inferred to be $171^{+11}_{-11}$ km s$^{-1}$ in the direction $l=301^{\circ} \pm 4^{\circ}$ and $b=0^{\circ} \pm 3^{\circ}$. We obtain $f\sigma_{8} = 0.400 \pm 0.017$, equivalent to $S_8 \approx \sigma_8(\Omega_m/0.3)^{0.55}=0.776\pm0.033$, which corresponds to an approximately $ 4\%\,$ statistical uncertainty on the value of $f\sigma_8$. Our inferred value is consistent with other low redshift results in the literature.

==> sections/A2.tex <==
\section{Second amendment catalogue}\label{sec:A2_data}

We are publishing along with this paper the second amendment catalogue of supernovae that we compiled and used for our peculiar velocity study. The first few entries of the catalogue are presented in Table \ref{tbl:A2_cat}. The distance modulus and its uncertainty for the LOSS and the Foundation catalogues are calculated using the best fit parameters, $M, \alpha, \mathcal{B}, \sigma_{\text{int}}$ inferred using the Forward likelihood method.


%\begin{landscape}
%\end{landscape}
